RF pulse shaping for gated electron mirrors

We present the design and prototype of a switchable electron mirror, along with a technique for driving it with a flat-top pulse. We employ a general technique for electronic pulse-shaping, where high fidelity of the pulse shape is required but the characteristics of the system, which are possibly nonlinear, are not known. This driving technique uses an arbitrary waveform generator to pre-compensate the pulse, with a simple iterative algorithm used to generate the input waveform. We demonstrate improvement in RMS error of roughly two orders of magnitude over an uncompensated waveform. This is a broadly applicable, general method for arbitrary pulse shaping.

==> tex/data_availability.tex <==
\section*{Data Availability}
The data that support the findings of this study are available from the corresponding author upon reasonable request.


==> tex/preamble.tex <==
\input{tex/\template} %
\usepackage{graphicx}%
\usepackage{dcolumn}%
\usepackage{bm}%

\usepackage{import} %
\usepackage{siunitx}
\usepackage{hyperref}
\usepackage{float}
\usepackage{amssymb} %

\newcommand{\naive}{na\"ive}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\insitu}{\emph{in situ}}

\RequirePackage[usenames,dvipsnames]{xcolor}
\newcommand{\fixme}[1]{{\bf \emph{\color{green} FIXME: \color{Fuchsia} #1}}}

\usepackage{flushend}

\usepackage{ifthen}

\newcommand{\paper}{Manuscript}

\newcommand{\ansys}{Ansys HFSS}

\newcommand{\Lsone}{Solid blue}
\newcommand{\Lstwo}{Dashed black}
\newcommand{\Lsthree}{Dotted red}
\newcommand{\lsone}{solid blue}
\newcommand{\lstwo}{dashed black}
\newcommand{\lsthree}{dotted red}

\usepackage{tikz}
\usetikzlibrary{shapes.geometric, arrows, arrows.meta}

\newcommand{\residcolor}{red}
\newcommand{\flowchartresidnoun}{dotted red box}
\newcommand{\measurecolor}{green}
\newcommand{\flowchartmeasurenoun}{green ellipse}
\newcommand{\yawgcolor}{blue}
\newcommand{\flowchartyawgnoun}{dashed blue box}

\newcommand{\pluseq}{\mathrel{+}=}

\ifthenelse{\equal{\template}{rsi}}{\newcommand{\ifrsi}[1]{#1}}{\newcommand{\ifrsi}[1]{}}
\newcommand{\mmview}{\ifrsi{ (Multimedia view)}}

\renewcommand*{\figureautorefname}{Fig.}

